Faster Discovery of Faster System Configurations with Spectral Learning

Despite the huge spread and economical importance of configurable software systems, there is unsatisfactory support in utilizing the full potential of these systems with respect to finding performance-optimal configurations. Prior work on predicting the performance of software configurations suffered from either (a) requiring far too many sample configurations or (b) large variances in their predictions. Both these problems can be avoided using the WHAT spectral learner. WHAT's innovation is the use of the spectrum (eigenvalues) of the distance matrix between the configurations of a configurable software system, to perform dimensionality reduction. Within that reduced configuration space, many closely associated configurations can be studied by executing only a few sample configurations. For the subject systems studied here, a few dozen samples yield accurate and stable predictors - less than 10% prediction error, with a standard deviation of less than 2%. When compared to the state of the art, WHAT (a) requires 2 to 10 times fewer samples to achieve similar prediction accuracies, and (b) its predictions are more stable (i.e., have lower standard deviation). Furthermore, we demonstrate that predictive models generated by WHAT can be used by optimizers to discover system configurations that closely approach the optimal performance.

==> Makefile <==
Src=tuningpredictor
Name=15tune
Bib=tuningpredictor.bib

all : dirs tex bib  tex tex embedfonts done


publish : dirs all
	cp $(HOME)/tmp/$(Src).pdf pdf/$(Name).pdf
	chmod a+r pdf/$(Name).pdf
	scp -p pdf/$(Name).pdf stuff@ttoy.net:menzies.us/pdf

commit:; - git status; git commit -a; git push origin master
typo:  ; - git status; git commit -am "typo"; git push origin master
update:; - git pull origin master
status:; - git status
gitting:
	git config --global credential.helper cache
	git config credential.helper 'cache --timeout=3600'

preview:
	open $(HOME)/tmp/$(Src).pdf &

view :
	evince $(HOME)/tmp/$(Src).pdf &

one : dirs tex done 

ready :
	mkdir -p $(HOME)/tmp

done :
	@printf "\n\n\n==============================================\n"
	@printf       "see output in $(HOME)/tmp/$(Src).pdf\n"
	@printf       "==============================================\n\n\n"
	@printf "\n\nWarnings (may be none):\n\n"
	grep arning $(HOME)/tmp/${Src}.log

dirs : 
	- [ ! -d $(HOME)/tmp ] && mkdir $(HOME)/tmp
	- [ ! -d pdf ] && mkdir pdf

tex : ready
	- pdflatex --shell-escape -output-directory=$(HOME)/tmp $(Src)

embedfonts:
	@ gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite \
          -sOutputFile=$(HOME)/tmp/$(Src)-embedded.pdf $(HOME)/tmp/$(Src).pdf
	@ mv              $(HOME)/tmp/$(Src)-embedded.pdf $(HOME)/tmp/$(Src).pdf

bib : 
	- cp $(Bib) $(HOME)/tmp; cd $(HOME)/tmp; bibtex $(Src)


==> activeconfig (1)/Makefile <==
Src=tuningpredictor
Name=15tune
Bib=tuningpredictor.bib

all : dirs tex bib  tex tex embedfonts done


publish : dirs all
	cp $(HOME)/tmp/$(Src).pdf pdf/$(Name).pdf
	chmod a+r pdf/$(Name).pdf
	scp -p pdf/$(Name).pdf stuff@ttoy.net:menzies.us/pdf

commit:; - git status; git commit -a; git push origin master
typo:  ; - git status; git commit -am "typo"; git push origin master
update:; - git pull origin master
status:; - git status
gitting:
	git config --global credential.helper cache
	git config credential.helper 'cache --timeout=3600'

preview:
	open $(HOME)/tmp/$(Src).pdf &

view :
	evince $(HOME)/tmp/$(Src).pdf &

one : dirs tex done 

ready :
	mkdir -p $(HOME)/tmp

done :
	@printf "\n\n\n==============================================\n"
	@printf       "see output in $(HOME)/tmp/$(Src).pdf\n"
	@printf       "==============================================\n\n\n"
	@printf "\n\nWarnings (may be none):\n\n"
	grep arning $(HOME)/tmp/${Src}.log

dirs : 
	- [ ! -d $(HOME)/tmp ] && mkdir $(HOME)/tmp
	- [ ! -d pdf ] && mkdir pdf

tex : ready
	- pdflatex --shell-escape -output-directory=$(HOME)/tmp $(Src)

embedfonts:
	@ gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite \
          -sOutputFile=$(HOME)/tmp/$(Src)-embedded.pdf $(HOME)/tmp/$(Src).pdf
	@ mv              $(HOME)/tmp/$(Src)-embedded.pdf $(HOME)/tmp/$(Src).pdf

bib : 
	- cp $(Bib) $(HOME)/tmp; cd $(HOME)/tmp; bibtex $(Src)

